Motion-based extrinsic sensor-to-sensor calibration: Effect of reference frame selection for new and existing methods

This paper studies the effect of reference frame selection in sensor-to-sensor extrinsic calibration when formulated as a motion-based hand-eye calibration problem. Different reference selection options are tested under varying noise conditions in simulation, and the findings are validated with real data from the KITTI dataset. We propose two nonlinear cost functions for optimization and compare them with four state-of-the-art methods. One of the proposed cost functions incorporates outlier rejection to improve calibration performance and was shown to significantly improve performance in the presence of outliers, and either match or outperform the other algorithms in other noise conditions. However, the performance gain from reference frame selection was deemed larger than that from algorithm selection. In addition, we show that with realistic noise, the reference frame selection method commonly used in literature is inferior to other tested options, and that relative error metrics are not reliable for telling which method achieves best calibration performance.

==> tables/Ali_kitti_keyframe.tex <==
\begin{table}[H]
\centering
\caption{Camera to lidar calibration on \textnormal{\texttt{2011\_09\_30\_drive\_0027}} using Ali~\citep{Ali2019}}
\label{tab:camLidarAli}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
Ali A & 0.935 & 2.445 & 24.598 & 1.863 \\
Ali B1 & \bfseries 0.042 & \bfseries 0.111 & 0.630 & \bfseries 0.666 \\
Ali B5 & 0.170 & 0.294 & \bfseries 0.342 & 0.722 \\
Ali B10 & 0.298 & 0.487 & 0.388 & 0.778 \\
Ali C5 & 0.088 & 0.192 & 0.749 & 1.075 \\
Ali C10 & 0.162 & 0.273 & 0.658 & 0.764 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Ali_kitti_long_cam.tex <==
\begin{table}[H]
\centering
\caption{Camera to camera calibration on \textnormal{\texttt{2011\_10\_03\_drive\_0027}} using Ali~\citep{Ali2019}}
\label{tab:camCamAli}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
Ali A & 4.668 & 0.533 & 43.137 & 0.366 \\
Ali B1 & \bfseries 0.034 & \bfseries 0.139 & 0.178 & 0.450 \\
Ali B5 & 0.155 & 0.181 & \bfseries 0.074 & 0.432 \\
Ali B10 & 0.305 & 0.205 & 0.117 & 0.435 \\
Ali C5 & 0.076 & 0.149 & 0.513 & 0.421 \\
Ali C10 & 0.153 & 0.169 & 0.210 & \bfseries 0.342 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/DNLO_kitti_keyframe.tex <==
\begin{table}[H]
\centering
\caption{Camera to lidar calibration on \textnormal{\texttt{2011\_09\_30\_drive\_0027}} using DNLO}
\label{tab:camLidarDNLO}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
DNLO A & 0.926 & 2.355 & 8.299 & 1.755 \\
DNLO B1 & \bfseries 0.038 & \bfseries 0.112 & 0.330 & 0.441 \\
DNLO B5 & 0.151 & 0.290 & 0.837 & 0.233 \\
DNLO B10 & 0.271 & 0.488 & \bfseries 0.202 & 0.232 \\
DNLO C5 & 0.079 & 0.187 & 0.486 & 0.757 \\
DNLO C10 & 0.144 & 0.265 & 0.300 & \bfseries 0.219 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/DNLO_kitti_long_cam.tex <==
\begin{table}[H]
\centering
\caption{Camera to camera calibration on \textnormal{\texttt{2011\_10\_03\_drive\_0027}} using DNLO}
\label{tab:camCamDNLO}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
DNLO A & 4.882 & 0.539 & 41.895 & 0.454 \\
DNLO B1 & \bfseries 0.034 & \bfseries 0.139 & 0.194 & 0.416 \\
DNLO B5 & 0.156 & 0.182 & 0.190 & 0.459 \\
DNLO B10 & 0.306 & 0.205 & 0.381 & 0.434 \\
DNLO C5 & 0.076 & 0.149 & \bfseries 0.159 & \bfseries 0.345 \\
DNLO C10 & 0.152 & 0.168 & 0.203 & 0.407 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/DNL_kitti_keyframe.tex <==
\begin{table}[H]
\centering
\caption{Camera to lidar calibration on \textnormal{\texttt{2011\_09\_30\_drive\_0027}} using DNL}
\label{tab:camLidarDNL}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
DNL A & 0.935 & 2.445 & 24.598 & 1.863 \\
DNL B1 & \bfseries 0.042 & \bfseries 0.111 & 0.629 & \bfseries 0.669 \\
DNL B5 & 0.170 & 0.293 & \bfseries 0.342 & 0.721 \\
DNL B10 & 0.298 & 0.487 & 0.388 & 0.777 \\
DNL C5 & 0.088 & 0.188 & 0.750 & 0.996 \\
DNL C10 & 0.162 & 0.273 & 0.658 & 0.764 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/DNL_kitti_long_cam.tex <==
\begin{table}[H]
\centering
\caption{Camera to camera calibration on \textnormal{\texttt{2011\_10\_03\_drive\_0027}} using DNL}
\label{tab:camCamDNL}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
DNL A & 4.668 & 0.533 & 43.137 & 0.366 \\
DNL B1 & \bfseries 0.034 & \bfseries 0.139 & 0.178 & 0.450 \\
DNL B5 & 0.155 & 0.181 & \bfseries 0.074 & 0.432 \\
DNL B10 & 0.305 & 0.205 & 0.117 & 0.435 \\
DNL C5 & 0.076 & 0.149 & 0.513 & 0.416 \\
DNL C10 & 0.153 & 0.169 & 0.210 & \bfseries 0.343 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Park_kitti_keyframe.tex <==
\begin{table}[H]
\centering
\caption{Camera to lidar calibration on \textnormal{\texttt{2011\_09\_30\_drive\_0027}} using Park~\citep{Park2020}}
\label{tab:camLidarPark}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
Park A & 17.068 & 1.939 & 30.581 & 16.190 \\
Park B1 & \bfseries 0.043 & \bfseries 0.110 & 0.618 & 0.747 \\
Park B5 & 0.160 & 0.286 & 0.368 & \bfseries 0.568 \\
Park B10 & 0.325 & 0.473 & \bfseries 0.183 & 0.849 \\
Park C5 & 0.087 & 0.165 & 0.903 & 0.623 \\
Park C10 & 0.254 & 0.260 & 2.179 & 1.586 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Park_kitti_long_cam.tex <==
\begin{table}[H]
\centering
\caption{Camera to camera calibration on \textnormal{\texttt{2011\_10\_03\_drive\_0027}} using Park~\citep{Park2020}}
\label{tab:camCamPark}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
Park A & 11.369 & 0.497 & 101.102 & 3.123 \\
Park B1 & \bfseries 0.034 & \bfseries 0.139 & 0.189 & 0.425 \\
Park B5 & 0.157 & 0.181 & \bfseries 0.078 & 0.351 \\
Park B10 & 0.309 & 0.204 & 0.145 & 0.347 \\
Park C5 & 0.076 & 0.149 & 0.515 & 0.399 \\
Park C10 & 0.154 & 0.168 & 0.255 & \bfseries 0.342 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Taylor_kitti_keyframe.tex <==
\begin{table}[H]
\centering
\caption{Camera to lidar calibration on \textnormal{\texttt{2011\_09\_30\_drive\_0027}} using Taylor~\citep{Taylor2015}}
\label{tab:camLidarTaylor}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
Taylor A & 17.068 & 1.939 & 30.581 & 16.190 \\
Taylor B1 & \bfseries 0.043 & \bfseries 0.110 & 0.618 & 0.747 \\
Taylor B5 & 0.160 & 0.286 & 0.368 & \bfseries 0.568 \\
Taylor B10 & 0.325 & 0.473 & \bfseries 0.183 & 0.849 \\
Taylor C5 & 0.087 & 0.165 & 0.903 & 0.623 \\
Taylor C10 & 0.254 & 0.260 & 2.179 & 1.586 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Taylor_kitti_long_cam.tex <==
\begin{table}[H]
\centering
\caption{Camera to camera calibration on \textnormal{\texttt{2011\_10\_03\_drive\_0027}} using Taylor~\citep{Taylor2015}}
\label{tab:camCamTaylor}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
Taylor A & 11.369 & 0.497 & 101.102 & 3.123 \\
Taylor B1 & \bfseries 0.034 & \bfseries 0.139 & 0.189 & 0.425 \\
Taylor B5 & 0.157 & 0.181 & \bfseries 0.078 & 0.351 \\
Taylor B10 & 0.309 & 0.204 & 0.145 & 0.347 \\
Taylor C5 & 0.076 & 0.149 & 0.515 & 0.399 \\
Taylor C10 & 0.154 & 0.168 & 0.255 & \bfseries 0.342 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Zhuang_kitti_keyframe.tex <==
\begin{table}[H]
\centering
\caption{Camera to lidar calibration on \textnormal{\texttt{2011\_09\_30\_drive\_0027}} using Zhuang~\citep{Zhuang1994}}
\label{tab:camLidarZhuang}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
Zhuang A & 0.973 & 2.405 & 23.339 & 1.789 \\
Zhuang B1 & \bfseries 0.055 & \bfseries 0.152 & \bfseries 1.063 & 2.899 \\
Zhuang B5 & 0.187 & 0.475 & 2.610 & 2.357 \\
Zhuang B10 & 0.323 & 0.542 & 3.840 & \bfseries 1.026 \\
Zhuang C5 & 0.094 & 0.279 & 1.439 & 2.643 \\
Zhuang C10 & 0.174 & 0.340 & 2.117 & 1.297 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Zhuang_kitti_long_cam.tex <==
\begin{table}[H]
\centering
\caption{Camera to camera calibration on \textnormal{\texttt{2011\_10\_03\_drive\_0027}} using Zhuang~\citep{Zhuang1994}}
\label{tab:camCamZhuang}
\begin{tabular}{lS[table-format=1.3]S[table-format=1.3]S[table-format=1.3]S[table-format=1.3]}
\toprule
{} & \multicolumn{2}{c}{Relative error} & \multicolumn{2}{c}{Absolute error} \\
{Method} & {$e_{rt}$ (m)} & {$e_{rR}$ (deg)} & {$e_{at}$ (m)} & {$e_{aR}$ (deg)} \\
\midrule
Zhuang A & 4.668 & 0.533 & 43.137 & 0.366 \\
Zhuang B1 & \bfseries 0.034 & \bfseries 0.139 & 0.180 & \bfseries 0.319 \\
Zhuang B5 & 0.155 & 0.181 & \bfseries 0.074 & 0.400 \\
Zhuang B10 & 0.305 & 0.205 & 0.117 & 0.430 \\
Zhuang C5 & 0.076 & 0.149 & 0.513 & 0.367 \\
Zhuang C10 & 0.153 & 0.169 & 0.210 & 0.329 \\
\bottomrule
\end{tabular}
\end{table}

